Examining user reviews of conversational systems: a case study of Alexa skills

Conversational systems use spoken language to interact with their users. Although conversational systems, such as Amazon Alexa, are becoming common and afford interesting functionalities, there is little known about the issues users of these systems face. In this paper, we study user reviews of more than 2,800 Alexa skills to understand the characteristics of the reviews and issues that are raised in them. Our results suggest that most skills receive less than 50 reviews. Our qualitative study of user reviews using open coding resulted in identifying 16 types of issues in the user reviews. Issues related to the content, integration with online services and devices, error, and regression are top issues raised by the users. Our results also indicate differences in volume and types of complaints by users when compared with more traditional mobile applications. We discuss the implication of our results for practitioners and researchers.

==> RQ1.tex <==
- Review Statistics: Number, size and  distribution of received reviews per App and per category.  
  - Statistics about sample sentences: number, size of sample sentences, semantic overlap between them. 
  - Time distribution of reviews.
  -  User specific statistics, e.g., users' average review, users' average review per App and per category. 
 -  Topic modeling and sentiment analysis of reviews.
 - Topic modeling of the  description of Apps.
 
 
 
 Results:
 The following is a brief summary of some exploratory analyses.
·     Most apps have less than 50 reviews. 
·     The average size of reviews is less than 250 for most apps.
·     Among apps Streaming services, Smart home and Games have the highest number of reviews. 
·     There is much variation in the average size of reviews per category. 
·     The average size of reviews for Currency guides & Converters, Taxi & Ridesharing, Connected Car, Smart Home and Social Networking are the highest among other apps.
·     Number of sentences (commands) for most of the apps is 13.
·     Average size of sentences (commands) is less than 10 for most of the apps.
·     Most reviews are from the time period between 2017 and 2018.
·     Most of the users have put less than 3 reviews.

==> TODO.tex <==
31) Complaint table
2) Comparing our results with Ahmed Hassan paper's results
3) Writing about implementing an Alexa skill Done
4) Scrape the skills again using the provided scripts - Andrew
5) Scrape Alexa devices, filter those related to skills - Andrew
(Overview\_AlexaSkill)

Crawler Options:
[Alexa Crawler] [D] What do you want to do?
[Alexa Crawler] [D] 1 - Scrap data from a specific category
[Alexa Crawler] [D] 2 - Scrap random pages from random categories
[Alexa Crawler] [D] 3 - Scrap from a specific app
[Alexa Crawler] [D] 0 - Exit


==> alexa-overview.tex <==
\subsection*{Implementing and Deploying an Alexa skill}
Developing an Alexa skill contains three parts: 1) creating and configuring Amazon Developer account for creating Alexa skills 2) creating and configuring Amazon Web Services account for hosting the skill on lambda 3) Writing code for the skill that can be done in two ways. Writing code on the AWS lambda console or writing code on the local server and uploading on the lambda (using ASK SDK for Python which is skill development kit). For having interactions with the skill, a skill needs to respond to events which is sent to the skill. So, by using SDK packages writing request handlers are possible which can handle requests and providing responses. Finally, a lambda function should be created, and code can be prepared for uploading on the lambda function (if code is on the local server). 

==> codes.tex <==
\begin{table*}
\caption{Type of complaints in reviews of Alexa Skills}
\begin{tabular}{|c|p{5cm}|p{5cm}|} 
\hline
\end{tabular}
\end{table*}

==> interesting.tex <==
\Fix{Interesting quotes}

\begin{quote}
    Too wordy. Need to simplify commands.
\end{quote}

\begin{quote}
    Alexa crashes after 3 questions
\end{quote}

\begin{quote}
    Can not stop it from playing.
\end{quote}

\begin{quote}
    always a day behind on news
\end{quote}

\begin{quote}
    Why? Distracting! Get rid of the music!
\end{quote}

\begin{quote}
    Voice commands is very hit and miss.
\end{quote}

\begin{quote}
    Would not recognize "Eleven Biotheraputics" or "Antero Resources"
\end{quote}

\begin{quote}
    Too hard to understand what is being asked.
\end{quote}

\begin{quote}
    Inconsistent response time.  Sometimes it works sometimes it doesn't.
\end{quote}

\begin{quote}
    I didn't like the joke. they were dark jokes.
\end{quote}

\begin{quote}
    This is good when it works.  Keeps quitting. Please fix it.
\end{quote}

\begin{quote}
    Very buggy, doesn't recognize the choices I'm making and keeps restarting to demo. Good idea but very poorly executed.
\end{quote}

\begin{quote}
    It probably works very well. Problem Alexa has issues understanding American English.  If you speak slow and slower.  It does the function. But listening is degrading on my alexa...
\end{quote}

\begin{quote}
    I have been listening to Forest Night for almost a year now.  It WAS my absolute favorite! What happened over the weekend??  Where did the owl go??  Why is the volume so much louder??  This isn't an improvement!! Now Forest Night is just another cricket infested sound loop.  I'm so disappointed.
\end{quote}

\begin{quote}
    Alexa always tells me that there was a problem with the command that I send, but it ultimately does it. Also, 100\% of the time Alexa thinks that I am talking about the LEXUS skill, not Linksys. I always have to really exaggerate the word Linksys in order to get the correct skill.
\end{quote}

\begin{quote}
    this is fun when you have absolutely no chance of interuption. When this is open, and I say Alexa End, this skill first confirms I want to close, then asks me to give feedback, then suggest other skills; when i angrily scream ALEXA END ALEXA END TRIVIA HERO I am told she didnt get that.
\end{quote}

\begin{quote}
    First, you have to remember the exact wording, phrase, I think even attitude when you're issuing a command or it will not do it.  Second, if you try to disarm the system it will ask you to generate a pin. Problem is there's nowhere to do that, not even in the skill settings
\end{quote}

\begin{quote}
    We have constantly failed to ask alexa to open/close garage door when we first say it because most of the time it doesnt understand “smart meross” You have to say it in a special way. We haven’t exactly figured out the right enounciation. Anyways, please consider using shorter and easier keyword for the skill.
\end{quote}

\begin{quote}
    This skill is simple and nice. Basically just what you want. Except... as you're trying to lull to sleep and say goodnight, you get the little response followed by a 15 second equivalent of yelling "leave a review and smash that like button!!!1!". Obviously this ruins the good night mood. Removing the review begging would make this a 4-5 star skill.
\end{quote}

\begin{quote}
    This is great EXCEPT for the requirement to say Amen after every Hail Mary. Alexa doesn’t accept my Amen 30\% of the time, which causes many annoying interruptions in my rosary. It would be much better if the rosary would continue without stopping. Please fix this skill. I would use it almost daily if it worked. I would really like a Rosary skill.
\end{quote}


\begin{quote}
    They’ve changed the format so many times at this point that my kids are frustrated. I don’t understand what was wrong with the original format. Since then we’ve introduced main stream characters my kids don’t know (they’re little) and can’t understand (Bane). We finally smoothed that out with a review of the word after a little storyline. Now we’re doing an Irish accent sped up so they can’t understand anything. I’m about to cut this from our morning routine.
\end{quote}

\begin{quote}
    I have Multiple Sclerosis so I was very excited to add this app. I added my contacts and tested it out and it worked. My biggest issue with Alexa is that there are trigger words for apps. When I ordered Alexa with the hopes of it having abilities added like this, I had no idea I would have to remember trigger words for added capabilities especially in an emergency. Unless I practice these trigger words on a regular basis, I highly doubt I will remember them when needed the most. I keep trying to associate saying "Alexa ask my buddy..." with this emergency. Why is it not "Alexa I've fallen and I can't get up..." Or at least "Alexa I have an emergency..."
\end{quote}

\begin{quote}
    I loved this skill when it was first suggested to me, but this new True \& False only version sucks. It used to be great with intriguing questions and options to test your recall of history. Now it's always only true or false and I'm sorry but true and false was only every good for people taking tests that didn't know the answers and wanted a 50-50 chance. True \& false questions are boring and corrupting of your memory. It's basically asking am I telling a lie or not? Answer enough true or false questions and you may find yourself remembering a lie as a fact. Seems like a lazy way to toss in a bunch of new questions for the creators. I'll give this app a 5 star review if it goes back to its old version but this one is terrible. I don't intend on playing it anymore if it remains this way.
\end{quote}

\begin{quote}
    Mixed bag at this point.  Many long commands that could be shortened.  Also, can't seem to get Alexa to adjust the temperature of my spa.  I would think that would be a top level item.  What is the point of turning the spa on by voice if I have to go to a phone or computer to adjust the temperature?  I'd just do it all there.  I've asked for help and Alexa seems to get very confused, tells me I can ask for help, but won't give me a full list of skills, only 2 examples.
\end{quote}



==> recycle.tex <==

In this section we describe the implication of our findings
study particularly focus on the issues reported in the reviews by the users which are related to conversational systems (specifically Alexa skills). We also compare issues related to Mobile apps studied in the previous literature with our identified issues.
In this paper we study issues that users face while using conversational systems (specifically Alexa skills) to help developers and practitioners to realize the important parts in developing conversational systems which can lead to the user dissatisfaction.


%\input{alexa-overview.tex}
\begin{comment}

In Amazon Alexa ecosystem, the Skills are 
Thus can be  
user asks system to book flight from \textbf{San Francisco} to \textbf{France tomorrow}. In this example, "I want to book a flight from \textbf{San Francisco} to \textbf{France tomorrow}" is the utterance, booking of a flight is the intent and origin, destination and the date are our entities.



can have interactions with human via text and voice or both. These conversational systems consist of two categories: dialog agents and chatbots.
Dialog agents or task-oriented dialog agents interact with user and receive information during conversation which are needed for accomplishing a task/goal such as booking a flight.
\end{comment}


\begin{comment}

To specify an intent, developers needs to 

For instance, a skill user for booking hotel rooms can use the skill to make a reservation or cancel a reservation. Therefore,  making a reservation and canceling reservation are two intents that the Skill can expect in users' utterances.

% that is extracted by the conversational system from user utterance and system act upon it. 
For example, in a hotel reservation system, making new reservations and canceling an existing reservation are the intents that can occur in user's utterances, while 
check-in and checkout dates are entities that are necessary pieces of information for processing those utterances. 
To identify an intent, developers should provide a list of sample utterances pertaining to the intent, and the specify the entities in any. For example, the following can be a list of sample utterances for the room reservation intent. 
- book a room for the last week of December.\\ 
- reserve a room \\ 
- reserve a room from January 5th to January 8th.\\

Examples of these systems can be SIRI, Alexa, Google home, and etc.
Chatbots are intended to have casual, human characteristic conversations with users which are not goal-oriented and are designed to have an entertaining aspect (e.g., ELIZA 1966). Chatbots consists of two categories: rule-based chatbots (ELIZA) and corpus-based chatbots. In the rule-based approach, chatbot is trained based on some rules which is written by developers (XIML). In corpus-based approach system’s responses can be extracted from training corpus or another text. The corpus-based chatbots contain two approaches: IR-based approach and sequence to sequence approach (CNN). 

Short number of terms in conversational systems are the followings: intent, entity, utterance

\end{comment}


\begin{comment}
For the deployment of a skill, in addition to specifying the dialog, developers needs to configure servers and the services that should be activated in response to different user's intents. 
some of computations take place 
such as signal processing and speech to text activities, the logic

Developing an Alexa skill contains three parts: 1) creating and configuring Amazon Developer account for creating Alexa skills 2) creating and configuring Amazon Web Services account for hosting the skill on lambda 3) Writing code for the skill that can be done in two ways. Writing code on the AWS lambda console or writing code on the local server and uploading on the lambda (using ASK SDK for Python which is skill development kit). For having interactions with the skill, a skill needs to respond to events which is sent to the skill. So, by using SDK packages writing request handlers are possible which can handle requests and providing responses. Finally, a lambda function should be created, and code can be prepared for uploading on the lambda function (if code is on the local server). 


\end{comment}

==> results-old.tex <==
\section{results-old}



We did quantitative analyses on more than 10910 Alexa skills in 63 different categories. Results show that 
\observation{Most of the apps have fewer than 50 reviews.}
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\linewidth]{Distnumreviews.png}
    \caption{}
\label{fig:Distnumreviews}
\end{figure}
    

    
Most apps have an average review size of less than 250 characters (see figure ~\ref{fig:Dist-avg-size-reviews-app}) and 50 words (see figure ~\ref{fig:Distavgsizeword}).
The average size of reviews is about 110 character and 20 word for most of the apps. 

\observation{The average size of reviews is about 110 character and 20 word for most of the apps.}  
  
  \begin{figure}[!h]
  \centering
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{Dist-avg-size-reviews-app.png}
    \caption{}
  \label{fig:Dist-avg-size-reviews-app}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.37\textwidth}
    \includegraphics[width=\textwidth]{Distavgsizeword.png}
    \caption{}
  \label{fig:Distavgsizeword}
  \end{minipage}
\end{figure}
    
  
  
  
  
  
  
  
    
    
    


Among apps' categories Streaming services, Smart home and Games have the highest number of reviews (see figure ~\ref{fig:Num-reviews-category}).

\observation{Smart home and Games have the highest number of reviews }
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\linewidth]{Num-reviews-category.png}
    \caption{}
    \label{fig:Num-reviews-category}
    \end{figure}

There is much variation in average size of reviews per category. Figure  ~\ref{fig:avgsizereviewbyword} shows the average size of reviews for Currency guides \& Converters, Taxi \& Ride-sharing, Connected Car, Smart Home and Social Networking are the highest among other apps' categories.

    
\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\linewidth]{avgsizereviewbyword.png}
    \caption{}
    \label{fig:avgsizereviewbyword}
    \end{figure}    

    
      
    
    
\begin{figure}[!h]
  \centering
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{numCommand.png}
    \caption{}
  \label{fig:numCommand}
  \end{minipage}
  \hfill
  \begin{minipage}[b]{0.4\textwidth}
    \includegraphics[width=\textwidth]{sizeCommands.png}
    \caption{}
 \label{fig:sizeCommands}
  \end{minipage}
\end{figure}

    

Number of sentences (commands) for most of the apps is 13 
(see figure ~\ref{fig:numCommand}).
Average size of sentences (commands) is less than 10 words for most of the skills (cf. Figure ~\ref{fig:sizeCommands}).

\observation{Average size of sentences (commands) is less than 10 words for most of the skills}



Figure~\ref{fig:time} shows that most reviews are from the time period between 2017 and 2019. January of 2018 has the highest number of reviews.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.7\linewidth]{time.png}
    \caption{}
    \label{fig:time}
    \end{figure}

90\% %\Amin{The raw number does not provide sufficient insight into the size of this group. Percentage can be a better option. For example, ``86\% of users (more than 76000 users)''} 
  of users have put only one review (see figure \ref{fig:freqnumreviewuser}).

\begin{figure}%[h!]
    \centering
    \includegraphics[width=0.7\textwidth]{freqnumreviewuser.png}
    \caption{}
    \label{fig:freqnumreviewuser}
\end{figure}
    


Figure~\ref{fig:Rplot} illustrates that Streaming Services, Novelty and Humor and Games have the highest rating numbers (sum of number of people who have rated each category) among categories. 

\begin{figure}
\centering
\includegraphics[width=0.7\textwidth]{Rplot.png}
\caption{}
\label{fig:Rplot}
\end{figure}

There is also positive and significant correlation between number of reviews and average of star ratings. This shows in our data if the number of reviews increases the average of star ratings also will increase.

